Asymptotic Log-Det Rank Minimization via (Alternating) Iteratively Reweighted Least Squares

The affine rank minimization (ARM) problem is well known for both its applications and the fact that it is NP-hard. One of the most successful approaches, yet arguably underrepresented, is iteratively reweighted least squares (IRLS), more specifically $\mathrm{IRLS}$-$0$. Despite comprehensive empirical evidence that it overall outperforms nuclear norm minimization and related methods, it is still not understood to a satisfying degree. In particular, the significance of a slow decrease of the therein appearing regularization parameter denoted $\gamma$ poses interesting questions. While commonly equated to matrix recovery, we here consider the ARM independently. We investigate the particular structure and global convergence property behind the asymptotic minimization of the log-det objective function on which $\mathrm{IRLS}$-$0$ is based. We expand on local convergence theorems, now with an emphasis on the decline of $\gamma$, and provide representative examples as well as counterexamples such as a diverging $\mathrm{IRLS}$-$0$ sequence that clarify theoretical limits. We present a data sparse, alternating realization $\mathrm{AIRLS}$-$p$ (related to prior work under the name $\mathrm{SALSA}$) that, along with the rest of this work, serves as basis and introduction to the more general tensor setting. In conclusion, numerical sensitivity experiments are carried out that reconfirm the success of $\mathrm{IRLS}$-$0$ and demonstrate that in surprisingly many cases, a slower decay of $\gamma$ will yet lead to a solution of the ARM problem, up to the point that the exact theoretical phase transition for generic recoverability can be observed. Likewise, this suggests that non-convexity is less substantial and problematic for the log-det approach than it might initially appear.

==> tables/table_1_vector_by_p.tex <==
\definecolor{temporarytablecolor1}{RGB}{0,84,159}
\definecolor{temporarytablecolor2}{RGB}{142,163,190}
\definecolor{temporarytablecolor3}{RGB}{163,163,185}
\definecolor{temporarytablecolor4}{RGB}{181,160,176}
\definecolor{temporarytablecolor5}{RGB}{194,148,161}
\definecolor{temporarytablecolor6}{RGB}{161,16,53}
\begin{tabular}{ll||c |rcl|cc}
\multirow{2}{*}{instance} & \multicolumn{1}{r||}{ACM:} & $\mathcal{Q}_{\varepsilon} \in [0,0.98]$ & \multicolumn{3}{c|}{$\mathcal{Q}_{\varepsilon} \in (0.98,1.005)$} & $\mathcal{Q}_{\varepsilon} \in [1.005,\infty)$ & $\mathcal{Q}_{\varepsilon} = \infty$ \\
& \multicolumn{1}{r||}{recovery:} & \cross & \cross &  & \cmark & \multicolumn{2}{c}{\cross} \\
\hline
\hline
\multirow{6}{*}{${\ell = 50}$}
& {\color{temporarytablecolor1}$\bullet$} $p = 0.0$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{  0}{0} & \rcint{  0}{0} & \rcint{100}{0}  \\
& {\color{temporarytablecolor2}$\bullet$} $p = 0.2$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{  0}{0} & \rcint{  0}{0} & \rcint{100}{0}  \\
& {\color{temporarytablecolor3}$\bullet$} $p = 0.4$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{  0}{0} & \rcint{  0}{0} & \rcint{100}{0}  \\
& {\color{temporarytablecolor4}$\bullet$} $p = 0.6$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{  0}{0} & \rcint{  0}{0} & \rcint{100}{0}  \\
& {\color{temporarytablecolor5}$\bullet$} $p = 0.8$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{  0}{0} & \rcint{  0}{0} & \rcint{100}{0}  \\
& {\color{temporarytablecolor6}$\bullet$} $p = 1.0$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{  0}{0} & \rcint{  0}{0} & \rcint{100}{0}  \\
\hline
\multirow{6}{*}{${\ell = 60}$}
& {\color{temporarytablecolor1}$\bullet$} $p = 0.0$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcfloat{  0}{7} & \rcint{  0}{0} & \rcfloat{ 99}{3}  \\
& {\color{temporarytablecolor2}$\bullet$} $p = 0.2$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcfloat{  0}{6} & \rcint{  0}{0} & \rcfloat{ 99}{4}  \\
& {\color{temporarytablecolor3}$\bullet$} $p = 0.4$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcfloat{  0}{2} & \rcint{  0}{0} & \rcfloat{ 99}{8}  \\
& {\color{temporarytablecolor4}$\bullet$} $p = 0.6$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{  0}{0} & \rcint{  0}{0} & \rcint{100}{0}  \\
& {\color{temporarytablecolor5}$\bullet$} $p = 0.8$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{  0}{0} & \rcint{  0}{0} & \rcint{100}{0}  \\
& {\color{temporarytablecolor6}$\bullet$} $p = 1.0$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{  0}{0} & \rcint{  0}{0} & \rcint{100}{0}  \\
\hline
\multirow{6}{*}{${\ell = 70}$}
& {\color{temporarytablecolor1}$\bullet$} $p = 0.0$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcfloat{ 39}{6} & \rcint{  0}{0} & \rcfloat{ 60}{4}  \\
& {\color{temporarytablecolor2}$\bullet$} $p = 0.2$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{ 39}{0} & \rcint{  0}{0} & \rcint{ 61}{0}  \\
& {\color{temporarytablecolor3}$\bullet$} $p = 0.4$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcfloat{ 34}{7} & \rcint{  0}{0} & \rcfloat{ 65}{3}  \\
& {\color{temporarytablecolor4}$\bullet$} $p = 0.6$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcfloat{ 24}{9} & \rcint{  0}{0} & \rcfloat{ 75}{1}  \\
& {\color{temporarytablecolor5}$\bullet$} $p = 0.8$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcfloat{  8}{6} & \rcint{  0}{0} & \rcfloat{ 91}{4}  \\
& {\color{temporarytablecolor6}$\bullet$} $p = 1.0$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{  0}{0} & \rcint{  0}{0} & \rcint{100}{0}  \\
\hline
\multirow{6}{*}{${\ell = 80}$}
& {\color{temporarytablecolor1}$\bullet$} $p = 0.0$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcfloat{ 92}{1} & \rcint{  0}{0} & \rcfloat{  7}{9}  \\
& {\color{temporarytablecolor2}$\bullet$} $p = 0.2$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{ 93}{0} & \rcint{  0}{0} & \rcint{  7}{0}  \\
& {\color{temporarytablecolor3}$\bullet$} $p = 0.4$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcfloat{ 90}{3} & \rcint{  0}{0} & \rcfloat{  9}{7}  \\
& {\color{temporarytablecolor4}$\bullet$} $p = 0.6$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcfloat{ 86}{1} & \rcint{  0}{0} & \rcfloat{ 13}{9}  \\
& {\color{temporarytablecolor5}$\bullet$} $p = 0.8$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcfloat{ 66}{7} & \rcint{  0}{0} & \rcfloat{ 33}{3}  \\
& {\color{temporarytablecolor6}$\bullet$} $p = 1.0$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcfloat{  2}{3} & \rcint{  0}{0} & \rcfloat{ 97}{7}  \\
\hline
\multirow{6}{*}{${\ell = 90}$}
& {\color{temporarytablecolor1}$\bullet$} $p = 0.0$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcfloat{ 99}{8} & \rcint{  0}{0} & \rcfloat{  0}{2}  \\
& {\color{temporarytablecolor2}$\bullet$} $p = 0.2$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcfloat{ 99}{8} & \rcint{  0}{0} & \rcfloat{  0}{2}  \\
& {\color{temporarytablecolor3}$\bullet$} $p = 0.4$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcfloat{ 99}{8} & \rcint{  0}{0} & \rcfloat{  0}{2}  \\
& {\color{temporarytablecolor4}$\bullet$} $p = 0.6$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcfloat{ 99}{5} & \rcint{  0}{0} & \rcfloat{  0}{5}  \\
& {\color{temporarytablecolor5}$\bullet$} $p = 0.8$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcfloat{ 97}{9} & \rcint{  0}{0} & \rcfloat{  2}{1}  \\
& {\color{temporarytablecolor6}$\bullet$} $p = 1.0$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcfloat{ 35}{6} & \rcint{  0}{0} & \rcfloat{ 64}{4}  \\
\hline
\multirow{6}{*}{${\ell = 100}$}
& {\color{temporarytablecolor1}$\bullet$} $p = 0.0$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor2}$\bullet$} $p = 0.2$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor3}$\bullet$} $p = 0.4$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor4}$\bullet$} $p = 0.6$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor5}$\bullet$} $p = 0.8$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor6}$\bullet$} $p = 1.0$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcfloat{ 88}{2} & \rcint{  0}{0} & \rcfloat{ 11}{8}  \\
\end{tabular}


==> tables/table_1_vector_by_p_caption.tex <==
\def\temporarycaptioncommand{vector IRLS-${p}$ (gaussian, full, image method, {$n$} = 160, {$\#$}nonzero = 40)}

==> tables/table_2_matrix_by_p.tex <==
\definecolor{temporarytablecolor1}{RGB}{0,84,159}
\definecolor{temporarytablecolor2}{RGB}{142,163,190}
\definecolor{temporarytablecolor3}{RGB}{163,163,185}
\definecolor{temporarytablecolor4}{RGB}{181,160,176}
\definecolor{temporarytablecolor5}{RGB}{194,148,161}
\definecolor{temporarytablecolor6}{RGB}{161,16,53}
\begin{tabular}{ll||c |rcl|cc}
\multirow{2}{*}{instance} & \multicolumn{1}{r||}{ARM:} & $\mathcal{Q}_{\varepsilon} \in [0,0.98]$ & \multicolumn{3}{c|}{$\mathcal{Q}_{\varepsilon} \in (0.98,1.005)$} & $\mathcal{Q}_{\varepsilon} \in [1.005,\infty)$ & $\mathcal{Q}_{\varepsilon} = \infty$ \\
& \multicolumn{1}{r||}{recovery:} & \cross & \cross &  & \cmark & \multicolumn{2}{c}{\cross} \\
\hline
\hline
\multirow{6}{*}{${\ell = 63}$}
& {\color{temporarytablecolor1}$\bullet$} $p = 0.0$ & \rcfloat{ 15}{9} & \rcfloat{  4}{9} & + & \rcfloat{ 31}{9} & \rcfloat{ 11}{2} & \rcfloat{ 36}{1}  \\
& {\color{temporarytablecolor2}$\bullet$} $p = 0.2$ & \rcfloat{ 16}{2} & \rcfloat{  5}{1} & + & \rcint{ 34}{0} & \rcfloat{  8}{8} & \rcfloat{ 35}{9}  \\
& {\color{temporarytablecolor3}$\bullet$} $p = 0.4$ & \rcfloat{ 15}{9} & \rcfloat{  4}{6} & + & \rcfloat{ 32}{2} & \rcfloat{  5}{6} & \rcfloat{ 41}{7}  \\
& {\color{temporarytablecolor4}$\bullet$} $p = 0.6$ & \rcfloat{  9}{3} & \rcfloat{  2}{8} & + & \rcfloat{ 22}{4} & \rcfloat{  1}{6} & \rcfloat{ 63}{9}  \\
& {\color{temporarytablecolor5}$\bullet$} $p = 0.8$ & \rcfloat{  0}{3} & \rcint{  0}{0} & + & \rcfloat{  0}{2} & \rcint{  0}{0} & \rcfloat{ 99}{5}  \\
& {\color{temporarytablecolor6}$\bullet$} $p = 1.0$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{  0}{0} & \rcint{  0}{0} & \rcint{100}{0}  \\
\hline
\multirow{6}{*}{${\ell = 72}$}
& {\color{temporarytablecolor1}$\bullet$} $p = 0.0$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{ 99}{0} & \rcint{  0}{0} & \rcint{  1}{0}  \\
& {\color{temporarytablecolor2}$\bullet$} $p = 0.2$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{ 99}{0} & \rcint{  0}{0} & \rcint{  1}{0}  \\
& {\color{temporarytablecolor3}$\bullet$} $p = 0.4$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcfloat{ 98}{5} & \rcint{  0}{0} & \rcfloat{  1}{5}  \\
& {\color{temporarytablecolor4}$\bullet$} $p = 0.6$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcfloat{ 96}{5} & \rcint{  0}{0} & \rcfloat{  3}{5}  \\
& {\color{temporarytablecolor5}$\bullet$} $p = 0.8$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcfloat{ 49}{8} & \rcint{  0}{0} & \rcfloat{ 50}{2}  \\
& {\color{temporarytablecolor6}$\bullet$} $p = 1.0$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{  0}{0} & \rcint{  0}{0} & \rcint{100}{0}  \\
\hline
\multirow{6}{*}{${\ell = 108}$}
& {\color{temporarytablecolor1}$\bullet$} $p = 0.0$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor2}$\bullet$} $p = 0.2$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor3}$\bullet$} $p = 0.4$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor4}$\bullet$} $p = 0.6$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor5}$\bullet$} $p = 0.8$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor6}$\bullet$} $p = 1.0$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcfloat{ 98}{8} & \rcint{  0}{0} & \rcfloat{  1}{2}  \\
\end{tabular}


==> tables/table_2_matrix_by_p_caption.tex <==
\def\temporarycaptioncommand{matrix IRLS-${p}$ (gaussian, full, image method, ${\overline{n} = 12}$, ${\overline{r}_{\mathrm{rs}} = 3}$)}

==> tables/table_3_matrix_by_setting.tex <==
\definecolor{temporarytablecolor1}{RGB}{0,84,159}
\definecolor{temporarytablecolor2}{RGB}{64,127,183}
\definecolor{temporarytablecolor3}{RGB}{246,168,0}
\definecolor{temporarytablecolor4}{RGB}{250,190,80}
\definecolor{temporarytablecolor5}{RGB}{214,188,95}
\begin{tabular}{ll||c |rcl|cc}
\multirow{2}{*}{instance} & \multicolumn{1}{r||}{ARM:} & $\mathcal{Q}_{\varepsilon} \in [0,0.98]$ & \multicolumn{3}{c|}{$\mathcal{Q}_{\varepsilon} \in (0.98,1.005)$} & $\mathcal{Q}_{\varepsilon} \in [1.005,\infty)$ & $\mathcal{Q}_{\varepsilon} = \infty$ \\
& \multicolumn{1}{r||}{recovery:} & \cross & \cross &  & \cmark & \multicolumn{2}{c}{\cross} \\
\hline
\hline
\multirow{5}{*}{${\ell = 63}$}
& {\color{temporarytablecolor1}$\bullet$} gaussian (image) & \rcfloat{ 15}{9} & \rcfloat{  4}{9} & + & \rcfloat{ 31}{9} & \rcfloat{ 11}{2} & \rcfloat{ 36}{1}  \\
& {\color{temporarytablecolor2}$\bullet$} gaussian (relaxed) & \rcfloat{ 14}{9} & \rcfloat{  4}{9} & + & \rcfloat{ 31}{3} & \rcfloat{ 12}{1} & \rcfloat{ 36}{8}  \\
& {\color{temporarytablecolor3}$\bullet$} sampling (image) & \rcint{  8}{0} & \rcfloat{  4}{3} & + & \rcfloat{  5}{6} & \rcfloat{  0}{9} & \rcfloat{ 81}{2}  \\
& {\color{temporarytablecolor4}$\bullet$} sampling (relaxed) & \rcfloat{  7}{8} & \rcfloat{  4}{7} & + & \rcfloat{  5}{3} & \rcint{  1}{0} & \rcfloat{ 81}{2}  \\
& {\color{temporarytablecolor5}$\bullet$} sampling (alternating) & \rcfloat{  9}{2} & \rcfloat{  5}{5} & + & \rcint{  8}{0} & \rcfloat{  1}{1} & \rcfloat{ 76}{2}  \\
\hline
\multirow{5}{*}{${\ell = 72}$}
& {\color{temporarytablecolor1}$\bullet$} gaussian (image) & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{ 99}{0} & \rcint{  0}{0} & \rcint{  1}{0}  \\
& {\color{temporarytablecolor2}$\bullet$} gaussian (relaxed) & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcfloat{ 99}{1} & \rcint{  0}{0} & \rcfloat{  0}{9}  \\
& {\color{temporarytablecolor3}$\bullet$} sampling (image) & \rcfloat{  2}{4} & \rcint{  2}{0} & + & \rcfloat{ 77}{1} & \rcfloat{  0}{2} & \rcfloat{ 18}{3}  \\
& {\color{temporarytablecolor4}$\bullet$} sampling (relaxed) & \rcfloat{  2}{3} & \rcint{  2}{0} & + & \rcfloat{ 75}{9} & \rcfloat{  0}{2} & \rcfloat{ 19}{6}  \\
& {\color{temporarytablecolor5}$\bullet$} sampling (alternating) & \rcfloat{  2}{8} & \rcfloat{  2}{3} & + & \rcfloat{ 83}{3} & \rcint{  0}{0} & \rcfloat{ 11}{6}  \\
\hline
\multirow{5}{*}{${\ell = 108}$}
& {\color{temporarytablecolor1}$\bullet$} gaussian (image) & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor2}$\bullet$} gaussian (relaxed) & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor3}$\bullet$} sampling (image) & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor4}$\bullet$} sampling (relaxed) & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor5}$\bullet$} sampling (alternating) & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
\end{tabular}


==> tables/table_3_matrix_by_setting_caption.tex <==
\def\temporarycaptioncommand{matrix (A)IRLS-${0}$ by settings (${\overline{n} = 12}$, ${\overline{r}_{\mathrm{rs}} = 3}$)}

==> tables/table_4_alt_matrix_completion_r5_by_value.tex <==
\definecolor{temporarytablecolor1}{RGB}{208,188,97}
\definecolor{temporarytablecolor2}{RGB}{187,187,106}
\definecolor{temporarytablecolor3}{RGB}{167,186,114}
\definecolor{temporarytablecolor4}{RGB}{125,184,132}
\begin{tabular}{ll||c |rcl|cc}
\multirow{2}{*}{instance} & \multicolumn{1}{r||}{ARM:} & $\mathcal{Q}_{\varepsilon} \in [0,0.98]$ & \multicolumn{3}{c|}{$\mathcal{Q}_{\varepsilon} \in (0.98,1.005)$} & $\mathcal{Q}_{\varepsilon} \in [1.005,\infty)$ & $\mathcal{Q}_{\varepsilon} = \infty$ \\
& \multicolumn{1}{r||}{recovery:} & \cross & \cross &  & \cmark & \multicolumn{2}{c}{\cross} \\
\hline
\hline
\multirow{4}{*}{${c_{\mathrm{mf}} = 1.2}$}
& {\color{temporarytablecolor1}$\bullet$} $n = 50$, $\ell = 570$ & \rcint{ 12}{0} & \rcint{ 27}{0} & + & \rcint{ 59}{0} & \rcint{  0}{0} & \rcint{  2}{0}  \\
& {\color{temporarytablecolor2}$\bullet$} $n = 200$, $\ell = 2370$ & \rcint{ 14}{0} & \rcint{ 74}{0} & + & \rcint{  4}{0} & \rcint{  0}{0} & \rcint{  8}{0}  \\
& {\color{temporarytablecolor3}$\bullet$} $n = 500$, $\ell = 5970$ & \rcint{  4}{0} & \rcint{ 79}{0} & + & \rcint{  0}{0} & \rcint{  0}{0} & \rcint{ 17}{0}  \\
& {\color{temporarytablecolor4}$\bullet$} $n = 1000$, $\ell = 11970$ & \rcint{  0}{0} & \rcint{ 60}{0} & + & \rcint{  0}{0} & \rcint{  0}{0} & \rcint{ 40}{0}  \\
\hline
\multirow{4}{*}{${c_{\mathrm{mf}} = 1.6}$}
& {\color{temporarytablecolor1}$\bullet$} $n = 50$, $\ell = 760$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor2}$\bullet$} $n = 200$, $\ell = 3160$ & \rcint{  0}{0} & \rcint{  9}{0} & + & \rcint{ 91}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor3}$\bullet$} $n = 500$, $\ell = 7960$ & \rcint{  0}{0} & \rcint{ 32}{0} & + & \rcint{ 68}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor4}$\bullet$} $n = 1000$, $\ell = 15960$ & \rcint{  0}{0} & \rcint{ 56}{0} & + & \rcint{ 44}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
\hline
\multirow{4}{*}{${c_{\mathrm{mf}} = 2.0}$}
& {\color{temporarytablecolor1}$\bullet$} $n = 50$, $\ell = 950$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor2}$\bullet$} $n = 200$, $\ell = 3950$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor3}$\bullet$} $n = 500$, $\ell = 9950$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor4}$\bullet$} $n = 1000$, $\ell = 19950$ & \rcint{  0}{0} & \rcint{  4}{0} & + & \rcint{ 96}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
\end{tabular}


==> tables/table_4_alt_matrix_completion_r5_by_value_caption.tex <==
\def\temporarycaptioncommand{AIRLS-${0}$ (sampling, ${\overline{r}_{\mathrm{rs}} = 5}$)}

==> tables/table_5_alt_matrix_completion_r7_by_value.tex <==
\definecolor{temporarytablecolor1}{RGB}{208,188,97}
\definecolor{temporarytablecolor2}{RGB}{187,187,106}
\definecolor{temporarytablecolor3}{RGB}{167,186,114}
\definecolor{temporarytablecolor4}{RGB}{125,184,132}
\begin{tabular}{ll||c |rcl|cc}
\multirow{2}{*}{instance} & \multicolumn{1}{r||}{ARM:} & $\mathcal{Q}_{\varepsilon} \in [0,0.98]$ & \multicolumn{3}{c|}{$\mathcal{Q}_{\varepsilon} \in (0.98,1.005)$} & $\mathcal{Q}_{\varepsilon} \in [1.005,\infty)$ & $\mathcal{Q}_{\varepsilon} = \infty$ \\
& \multicolumn{1}{r||}{recovery:} & \cross & \cross &  & \cmark & \multicolumn{2}{c}{\cross} \\
\hline
\hline
\multirow{4}{*}{${c_{\mathrm{mf}} = 1.2}$}
& {\color{temporarytablecolor1}$\bullet$} $n = 50$, $\ell = 782$ & \rcint{  2}{0} & \rcint{  7}{0} & + & \rcint{ 91}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor2}$\bullet$} $n = 200$, $\ell = 3302$ & \rcint{  0}{0} & \rcint{ 66}{0} & + & \rcint{ 34}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor3}$\bullet$} $n = 500$, $\ell = 8342$ & \rcint{  0}{0} & \rcint{ 86}{0} & + & \rcint{ 13}{0} & \rcint{  0}{0} & \rcint{  1}{0}  \\
& {\color{temporarytablecolor4}$\bullet$} $n = 1000$, $\ell = 16742$ & \rcint{  0}{0} & \rcint{ 98}{0} & + & \rcint{  1}{0} & \rcint{  0}{0} & \rcint{  1}{0}  \\
\hline
\multirow{4}{*}{${c_{\mathrm{mf}} = 1.6}$}
& {\color{temporarytablecolor1}$\bullet$} $n = 50$, $\ell = 1042$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor2}$\bullet$} $n = 200$, $\ell = 4402$ & \rcint{  0}{0} & \rcint{  1}{0} & + & \rcint{ 99}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor3}$\bullet$} $n = 500$, $\ell = 11122$ & \rcint{  0}{0} & \rcint{  3}{0} & + & \rcint{ 97}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor4}$\bullet$} $n = 1000$, $\ell = 22322$ & \rcint{  0}{0} & \rcint{  5}{0} & + & \rcint{ 95}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
\hline
\multirow{4}{*}{${c_{\mathrm{mf}} = 2.0}$}
& {\color{temporarytablecolor1}$\bullet$} $n = 50$, $\ell = 1302$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor2}$\bullet$} $n = 200$, $\ell = 5502$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor3}$\bullet$} $n = 500$, $\ell = 13902$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor4}$\bullet$} $n = 1000$, $\ell = 27902$ & \rcint{  0}{0} & \rcint{  1}{0} & + & \rcint{ 99}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
\end{tabular}


==> tables/table_5_alt_matrix_completion_r7_by_value_caption.tex <==
\def\temporarycaptioncommand{AIRLS-${0}$ (sampling, ${\overline{r}_{\mathrm{rs}} = 7}$)}

==> tables/table_n1_matrix_conj.tex <==
\definecolor{temporarytablecolor1}{RGB}{0,84,159}
\definecolor{temporarytablecolor2}{RGB}{246,168,0}
\begin{tabular}{ll||c |rcl|cc}
\multirow{2}{*}{instance} & \multicolumn{1}{r||}{ARM:} & $\mathcal{Q}_{\varepsilon} \in [0,0.98]$ & \multicolumn{3}{c|}{$\mathcal{Q}_{\varepsilon} \in (0.98,1.005)$} & $\mathcal{Q}_{\varepsilon} \in [1.005,\infty)$ & $\mathcal{Q}_{\varepsilon} = \infty$ \\
& \multicolumn{1}{r||}{recovery:} & \cross & \cross &  & \cmark & \multicolumn{2}{c}{\cross} \\
\hline
\hline
\multirow{2}{*}{${\Delta\ell = -1}$}
& {\color{temporarytablecolor1}$\bullet$} gaussian & \rcfloat{ 46}{2} & \rcfloat{ 26}{5} & + & \rcint{  0}{0} & \rcfloat{ 20}{8} & \rcfloat{  6}{5}  \\
& {\color{temporarytablecolor2}$\bullet$} sampling & \rcfloat{ 20}{7} & \rcfloat{ 10}{3} & + & \rcint{  0}{0} & \rcfloat{  7}{2} & \rcfloat{ 61}{8}  \\
\hline
\multirow{2}{*}{${\Delta\ell = 0}$}
& {\color{temporarytablecolor1}$\bullet$} gaussian & \rcfloat{ 16}{7} & \rcfloat{  7}{1} & + & \rcint{ 34}{0} & \rcfloat{ 11}{6} & \rcfloat{ 30}{6}  \\
& {\color{temporarytablecolor2}$\bullet$} sampling & \rcint{ 10}{0} & \rcint{  6}{0} & + & \rcfloat{ 10}{1} & \rcfloat{  1}{4} & \rcfloat{ 72}{5}  \\
\hline
\multirow{2}{*}{${\Delta\ell = 1}$}
& {\color{temporarytablecolor1}$\bullet$} gaussian & \rcint{  0}{0} & \rcfloat{  0}{2} & + & \rcfloat{ 58}{2} & \rcfloat{  0}{1} & \rcfloat{ 41}{5}  \\
& {\color{temporarytablecolor2}$\bullet$} sampling & \rcfloat{  7}{4} & \rcfloat{  7}{2} & + & \rcfloat{ 22}{9} & \rcfloat{  0}{6} & \rcfloat{ 61}{9}  \\
\end{tabular}


==> tables/table_n1_matrix_conj_caption.tex <==
\def\temporarycaptioncommand{matrix IRLS-${0}$ (full, image method, ${\overline{n} = 12}$, ${\overline{r}_{\mathrm{rs}} = 3}$)}
